Characterizing the country-wide adoption and evolution of the Jodel messaging app in Saudi Arabia

Social media is subject to constant growth and evolution, yet little is known about their early phases of adoption. To shed light on this aspect, this paper empirically characterizes the initial and country-wide adoption of a new type of social media in Saudi Arabia that happened in 2017. Unlike established social media, the studied network Jodel is anonymous and location-based to form hundreds of independent communities country-wide whose adoption pattern we compare. We take a detailed and full view from the operators perspective on the temporal and geographical dimension on the evolution of these different communities -- from their very first the first months of establishment to saturation. This way, we make the early adoption of a new type of social media visible, a process that is often invisible due to the lack of data covering the first days of a new network.

==> template/journaldata.tex <==
\journaltitle      {The Journal of Web Science}
\journalshorttitle {JWS}
\journalurl        {webscience-journal.net}
\journalissnprint  {XXXX-XXXX}
\journalissnonline {XXXX-XXXX}
\journalaimsandscope{%
 This is a text to describe the aim of the journal\par
 \textit{\jws@journaltitle} is the name of the journal. \jws@journalshorttitle its short title.}
\journalsubmission{%
The \jws@journaltitle\ accepts only electronic submissions. See \jws@journalurl\ for complete instructions.}
\journalabstractedin{%
 Journal A, Journal B, Journal C}

